Model Tells You What to Discard: Adaptive KV Cache Compression for LLMs

In this study, we introduce adaptive KV cache compression, a plug-and-play method that reduces the memory footprint of generative inference for Large Language Models (LLMs). Different from the conventional KV cache that retains key and value vectors for all context tokens, we conduct targeted profiling to discern the intrinsic structure of attention modules. Based on the recognized structure, we then construct the KV cache in an adaptive manner: evicting long-range contexts on attention heads emphasizing local contexts, discarding non-special tokens on attention heads centered on special tokens, and only employing the standard KV cache for attention heads that broadly attend to all tokens. Moreover, with the lightweight attention profiling used to guide the construction of the adaptive KV cache, FastGen can be deployed without resource-intensive fine-tuning or re-training. In our experiments across various asks, FastGen demonstrates substantial reduction on GPU memory consumption with negligible generation quality loss. We will release our code and the compatible CUDA kernel for reproducibility.

==> TODO.tex <==
1. pruned ratio 是x 的情况下，方法 y 对于 attention map 的recover rate (on average of all heads) 是多少
2. evaluate un-adapted all-cache baseline
3. real-time throughput & memory & latency (integrated with DeepSpeed); 

==> input/ack.tex <==
\section*{Acknowledgement}
Here, we thank the helpful discussion with Jianwei Yang, ... 

==> old_abstract.tex <==
%% new version
In this study, we introduce adaptive KV cache compression, a plug-and-play method that reduces the memory footprint of generative inference for Large Language Models (LLMs) and accelerates its generation throughput. 
% accelerates the generation throughput of Large Language Models (LLMs) and reduces their memory footprint.
Different from conventional KV cache algorithms that retain key and value vectors for all context tokens, we conduct targeted profiling to discern the intrinsic structure of attention modules.
Based on the recognized structure, we then construct the KV cache in an adaptive manner: evicting long-range contexts on attention heads emphasizing local contexts, discarding non-special tokens on attention heads centered on special tokens, and only employing the standard KV cache for attention heads that broadly attend to all tokens.
Moreover, with the lightweight attention profiling used to guide the construction of the adaptive KV cache, \ours can be deployed without resource-intensive fine-tuning or re-training.
In our experiments across a diverse set of models and tasks, \ours demonstrates substantial efficiency enhancements on both GPU memory consumption and generation throughput. 

%% old version
% Large language models(LLMs) are powerful yet extremely expensive to conduct inference. Previously network compression techniques lower inference cost by trimming model size and compressing context length, but either requires expensive re-training or could significantly downgrade model quality. 
% In this work, we introduce KV-Malloc, an algorithm that provides a plug-in-and-play speed-up for any auto-regressive transformer-based language model. 
% KV-Malloc sparsifies KV caches by profiling each attention head based on its attention score distribution during decoding. 
% To do so, we design several sparse strategies summarized from empirical attention distribution, and select the most lossless strategy to prune the KV cache of each attention head.
% The strategy is decided only once based on the attention distribution of existing tokens at the beginning of generation, and persisted till the end of sentence, bringing little to no extra computation cost.
% We then empirically show that the method can preserve near-the-same performance while significantly reducing the memory footprints an computational cost on major foundational models across different generation tasks. 

% Addressing the prohibitively high inference cost associated with large language models (LLMs), particularly during the decoding of lengthy sequences, is a significant challenge. This is primarily due to the escalating memory required by the Key-Value (KV) cache, which grows linearly with sequence length, and the attention computation cost which goes quadratically. In this work, we propose a novel approach to optimize KV cache construction during decoding, thereby significantly reducing memory footprint and improving LLM throughput, without compromising model quality. Our approach draws on the observation that KV cache density is exceptionally high around the current decoding position but negligible elsewhere. We show both empirical and theoretical proof that storing only this peaking portion is sufficient, rendering it a significantly smaller cache. We then introduce an algorithm to determine whether a specific position in a given attention head meets the condition to trim. Notably, our model seamlessly integrates with any transformer-based language models without additional training requirements. We validate our algorithm on popular models including OPT, Llama2, and GPT-X across major benchmarks, showing substantial memory savings and speedup, while preserving comparable performance levels. 

==> old_intro.tex <==

% Large language models have brought foundational breakthrough to NLP research and industrial applications.
% These models advance various difficult tasks like open-domain chat, summarization, question answering to a level that we can hardly imagine a few years ago. Numerous big-techs and start-ups are eagerly to surf this trend by publishing their own LLM services.
% However, the inference cost for LLMs is also extremely expensive in both time and memory, making it challenging to guarantee a smooth experience in latency-sensitive applications. For example, while on average, a Google search takes 0.2 seconds, ChatGPT often requires 15-20 seconds or more, which gets worse when the generated sequence is longer.
% Also, transformer-based LLMs demand significant memory during inference for both model parameters and intermediate states, known as the KV cache.   
% For instance, the 540B Palm model, with a batch size of 512 and context length of 2048, needs 3TB for the KV cache. 
% The high memory footprints similarly constrains the throughput of the model, where bigger batch can easily overflow the best accelerators.
% As a result, how to optimize the inference of LLMs has attracted great attention. 

% Separately, another key observation from real-world is that, instead of applying the vanilla foundation models, both consumers and enterprises want a more personalized LLMs that better aligned with their own data and hardware. This leads to two requirements for the inference optimization algorithms. 
% (1) The algorithms have to be both model-agnostic and parameter-agnostic. The algorithms should be able to preserve LLM quality despite model choices and whether they are fine-tuned on domain spcific data.
% (2) The algorithms should be cheap to run. Ideally, the optimization shouldn't involve expensive retraining before deployment, nor increase computation cost while running.

% However, existing attempts in the literature can hardly satisfy all the requirements. 
% First, the most relevant works that directly tackles the KV cache problems, H2O, context pruning,gisting tokens, Lora, either requires re-training, or too expensive to deploy and could cause significant performance downgrade. 
% Second, the majority of earlier works focus on optimizing the encoding stage of the model, which cannot directly be adopted to the decoding part due to the left-to-right mask. 
% Lastly, works in quantization and distillation typically need training and could result in performance drop.
% -------------------------------------------------------

Large Language Models (LLMs) have revolutionized Natural Language Processing (NLP) research and industrial applications.
% , propelling advances in challenging tasks such as open-domain chat, summarization, and question answering. 
% Numerous companies, from big tech to startups, are racing to capitalize on this trend by offering their own LLM services.
However, the inference cost for LLMs remains a significant hurdle. At each decoding step, the key-value attention matrix for prompt and previously generated token, known as KV cache, has to be stored in memory to reduce repetitive operations.  
% For context, 
% while a Google search typically takes 0.2 seconds, a response from ChatGPT can often require 15-20 seconds, a delay that exacerbates as the generated sequence lengthens. 
% The substantial memory demands during inference—required both for model parameters and intermediate states (the KV cache)—are similarly problematic. 
For instance, the 540B Palm model, with a batch size of 512 and context length of 2048, requires a staggering 3TB for the KV cache. 
These memory requirements not only constrain model throughput, with large batches risking accelerator overflow, but they also challenge the timely and smooth deployment of these models in latency-sensitive applications.

Concurrently, there is a growing demand for more personalized LLMs that align better with users' unique data and hardware constraints, which generates hundreds thousands of model variations.
This desire translates into two non-trivial requirements for inference optimization algorithms:

1. Model and Parameter Agnostic: The algorithms must preserve LLM quality regardless of the model chosen and whether it has been fine-tuned on domain-specific data.\\
2. Cost-Efficient: Optimization should not necessitate expensive retraining before deployment or increase computational costs during operation.

Existing solutions in the literature, however, struggle to meet these criteria. 
For example, approaches like gisting tokens \citeauthor{gist} either demand re-training or are prohibitively expensive to deploy, with a potential for significant performance degradation. 
Moreover, most prior works are tailored to optimize the encoding stage of the model, which cannot be directly adapted for decoding due to the left-to-right masking constraint. 
Works in quantization and distillation often necessitate retraining and may result in a performance drop.

In summary, a pressing need exists for innovative inference optimization techniques suited for the decoding stage in LLMs—solutions that address these latency and throughput challenges without compromising on the two key criteria -outlined above.
Motivated by this, we propose KV-Malloc, a framework that dynamically plans KV cache quota for each attention head of any auto-regressive LLMs. 
Our method is based on 3 key observations, which we illustrate in \ref{fig:obs}.

\begin{figure}[t]
        \includegraphics[scale=0.4]{figures/Layer 77.pdf}

\caption{The left figure shows the sparsity of attention scores. The right figure illustrate how diverse each head is in terms of their attention score distribution patterns.}
\label{fig:obs}
\end{figure}

% First, the attention score during decoding could be very sparse. 
First, the KV cache could be highly sparse.
As shown in \ref{fig:att}, we observe that over $90\%$ mass of attention scores could falls in a (few) concentrated span of tokens that accounts for $10\%$ of the whole sequence. 
Similar phenomenon is also reported in \citeauthor{h2o}, \citeauthor{deja}.
The pattern indicates the possibility of more than 10 X reduction in cache size while preserving the matrix quality. 

% Second, not every attention head follows the same sparsity pattern. 
Second, the sparsity pattern is diverse for each attention head but could be classified into limited categories. 
We find that even for heads in the same layer, their attention scores could falls anywhere between extremely dense and extremely sparse. 
This indicates that we may personalize the compressing strategy for each attention head to best fit the actual distribution. 
Meanwhile, the personalization process should be very efficient to minimize the extra cost.

% Third, we both empirically and theoretically show the local density fading is a strong indicator of global sparsity. 
Third, we show it's sufficient to decide a satisficing strategy of the whole sequence for an attention head at the first decoding step.


% Taking \ref{fig:att} as an example, when decoding token i, we discover if the attention score near i - 2 and i + 2 approximate zero, then the head is very likely to have the sparsity pattern for the whole sequence decoding. 
% \ref{fig:att} shows how robust the indicator is on Llama, where we can see it has over $90\%$ recall and accuracy on classifying sparse heads.
% It inspires us to design a simple, yet effective algorithm to identify sparse heads from non-sparse heads.

Based on these observations, KV-Malloc has two stages: 
(1) calculate distribution profile of attention score for each head, 
(2) adaptively reduce the KV cache for each head given its distribution profile. 
More specifically, given the attention score distribution at the first step of decoding, KV-Malloc checks if the score for the first token in the sequence, namely the attention of the token being decoded, to the token representing the whole sentence, e.g., the first token in Llama, is high enough. 
If the score is higher than a given threshold, then KV-Malloc decides a strategy to evict the KV cache.
The default strategy will only leave KV cache for the first token, and the local tokens near the current decoding position.
Then we check if the lost rate is acceptable, by comparing the similarity of the trimmed cache and the original one.
If it's not acceptable, then KV-Malloc will adopt more comprehensive eviction policies like H20.
Note we only do (1) once, at the start of the decoding, for a whole sequence based on our third observation.

We evaluate the effectiveness of the framework on Llama and OPT, with a wide range of generative tasks from big-bench and lm-evaluation-harness. Our results demonstrate that:\\
(1) KV-Malloc can achieves X memory footprint reduction, Y throughput increase, Z latency reduction, compared to SOTA frameworks like H20 and DeepSpeed.\\
(2) KV-Malloc preserve the model quality better with the same cache budget, especially for fine-tuned models.




==> old_intro_new.tex <==

% Correspondingly, many attempts have been developed to accelerate the inference of large language models. 

Autoregressive language models that are based on the Transformer architecture have attracted extensive attention~\citep{openai2023gpt4,touvron2023llama}. 
Along with the increase of model size, these models present significant challenges in terms of computational workload and GPU memory consumption~\citet{540b}.
% Also, the remarkable success of these models across diverse applications underscores the pressing need for serving these models in an economically feasible manner.
Since these models achieve remarkable success across diverse applications, there is a pressing need for serving these models in an economically feasible manner.

% One emerging family of large Neural Network models is the Transformer-based autoregressive language models
% Leveraging these models for text generation typically involves deploying Key Value vectors cache mechanism, contributing to a large amount of GPU memory consumption. 
Leveraging these models for text generation involves using a Key-Value vectors cache mechanism (KV cache), which stores the key vectors and value vectors for all previous contexts, contributing significantly to GPU memory consumption. 
For instance, the 540B Palm model \citet{palm} requires a staggering 3TB KV cache for setting the batch size to 512 and the context length to 2048. 
Here, we propose \ours to \emph{accelerate the generative inference by compressing the KV cache in an adaptive manner}. 
\ours does not require any fine-tuning or re-training, thus can be applied in a plug-and-play manner. 


% it has been observed that implicit structure widely exists in the attention module, and not all tokens are necessary for all attention modules. 
Our study starts from the observation that 
there are abundant structures observed in attention modules\citep{sixteen, lift-prune,bert-look,structureprune,sparsetransformer}, and not all attention modules need to attend to all tokens \citep{deja,h2o,scissorhands}.
% can be discarded for some attention modules.
% Intuitively, it could greatly reduce memory consumption by introducing structure to the Key Value vectors cache and discarding unnecessary Key Value vectors. 
Intuitively, harvesting such structures and compressing cached vectors could substantially reduce memory consumption and accelerate text generation.
% Here, we propose FastGen, a profile-to-compress approach to construct adaptive LLM KV cache. 
Based on this intuition, \ours constructs an adaptive KV cache in a diagnose-to-compress manner. 
% Specifically, we develop an efficient profiling algorithm to recognize the structure of different attention modules, under the guidance of which, we construct the KV cache for different modules in an adaptive manner. 
% Specifically, we identify three frequent patterns in attention modules, i.e., some attention modules mostly attend to local contexts on which we construct KV cache that evicts long-range contexts, some mostly attend to certain tokens on which we construct KV cache that only retains special tokens, and some broadly attend to all tokens on which we employ the standard KV cache and store all tokens. 
First, we employ an efficient profiling algorithm to recognize the structural patterns for attention modules. 
Under the guidance of this profiling, we then construct the KV cache for various modules adaptively. 
\begin{figure}[t]
        \includegraphics[width=0.9\textwidth]{figures/profiles.png}
\caption{Diverse but Constrained Sparsity Pattern in Attention.}
\label{fig:obs}
\end{figure}

Specifically, \ours recognize four different attention structures and apply them correspondingly. 
Some attention modules mostly attend to local contexts, for which we construct a KV cache that evicts long-range contexts; some primarily attend to specific tokens, for which we create a KV cache that retains only special tokens; some have attention maps that are column-wise sparse, for which we discard the least frequently attended tokens; and some broadly attend to all tokens, for which we employ the standard KV cache and store all tokens.
In this way, our approach is able to compress the KV cache while retaining the original functionality of attention modules, thus accelerating text generation without the need for model re-training or fine-tuning.

% Applying \ours to a wide range of auro-regressive language models on various tasks, we observe that our method is able to accelerate text generation in a plug-and-play manner. 
We evaluate the effectiveness of the framework on Llama \citet{touvron2023llama} and OPT\citet{opt}, with a wide range of generative tasks from big-bench \citep{bigbench} and lm-evaluation-harness \citet{eval-harness}. Our results demonstrate that:
\begin{itemize}[leftmargin=*]
    \item
    \ours can achieves X memory footprint reduction, Y throughput increase, Z latency reduction, compared to SOTA frameworks like H20 and DeepSpeed.
    
    \item 
    \ours preserve the model quality better with the same cache budget, especially for fine-tuned models.
\end{itemize}



==> old_method.tex <==
\subsection{Problem Formulation}
In this section, we describe the general formulation of generative inference with multi-head attention and KV Cache.

\textbf{Multi-head Attention}

The transformer-decoder processes input sequences and generates tokens subsequently. 
Given a sequence of length n, where the first k tokens, $x_1,...,x_k$ are from the input, and the k+1 to n tokens, $x_{k+1}, ..., x_n$ are the decoding sequence. 
For the decoding step i, the sequence $x_1, ..., x_{k+i-1}$ are passed into the model and projected into the Q, K, V matrices. 
The query Q represent the position we want generate and the K, V matrices provide context information.
% To avoid recomputing the keys for each query, the keys and values for every item current in the sequence are cached in a key-value cache.
We then split $\mathbf{Q}, \mathbf{K}, \mathbf{V}$ into $h$ heads and perform scaled dot-product attention for each head:
\begin{align*}
\text{Attention}(\mathbf{Q}^h, \mathbf{K}^h, \mathbf{V}^h) = \softmax{\frac{\mathbf{Q}^h\mathbf{K}^{h \top}}{\sqrt{d_k}}}\mathbf{V}^h
\end{align*}

where $\mathbf{Q}^h, \mathbf{K}^h, \mathbf{V}h \in \mathbb{R}^{d_k \times n}$ and $d_k = d{model}/h$.

The attended values for each head are concatenated and projected to obtain $\mathbf{y}_i$, namely the multi-head attention(MHA).
We concatenate the attended values from each head and project with a matrix $\mathbf{W}^O$ to obtain the decoder output:

\begin{align*}
\mathbf{y}_i = [\text{Attention}_1(\mathbf{Q}_1, \mathbf{K}_1, \mathbf{V}_1); ... ; \text{Attention}^h(\mathbf{Q}^h, \mathbf{K}^h, \mathbf{V}^h)]\mathbf{W}^O
\end{align*}

\textbf{Key-value Cache}
In autoregressive decoding, the key and value matrices are based on the same partial sequence at each step i. Hence, we can cache the previous key and value matrices $\mathbf{K}{<i}, \mathbf{V}{<i}$ and reuse them when computing the attention at step i:

\begin{align*}
\mathbf{K} &= [\mathbf{K}_{<i}], \\
\mathbf{V} &= [\mathbf{V}{<i}],
\end{align*}

This caching reduces the computational cost, since $\mathbf{K}{<i}$ and $\mathbf{V}{<i}$ can be reused for every decoding step after the first one.

\subsection{KV-Malloc}
In this section, we introduce the KV-Malloc framework. 
KV-Malloc optimizes the attention distributions of each head during decoding to choose a customized sparse caching strategy for each head. 
Initially, attention distributions are profiled into predefined sparse patterns. 
We then simulate cache pruning for each head using various eviction policies, selecting the one that most closely aligns with the original cache. 

Let $A_{t}^h \in \mathbb{R}^{n \times n}$ be the attention distribution matrix for head $h$ at decoding timestep $t$, where $n$ is the input sequence length. 

For simplicity, we assume a set of $m$ predefined KV cache eviction policy $S = {S_1, ..., S_m}$. The implementation of each eviction policy will be discussed in the following section.
% where each $S_k \in {0, 1}^{n \times n}$ can be viewed as a binary mask.

For each head $h$, we select a policy $S_{h^*}$ by:

% $$S^{h^*} = \argmax_{h \in [1,m]} \text{sim}(A_{1}^h, S_k \odot A_{1}^h)$$
$$S^{h^*} = \argmax_{h \in [1,m]} \text{sim}(A_{1}^h, S_k(A_{1}^h))$$

where $\odot$ is elementwise multiplication and $\text{sim}(\cdot,\cdot)$ computes the cosine similarity between two matrices. 
This selects the policy with the highest similarity to the true attention for head $h$ at the first time step.

During decoding, the KV caches for head $h$ are then re-allocated as:

% $$\Tilde{K}^h = S^{h^*} \odot K^h, \quad \Tilde{V}^h = S^h \odot V^h$$
$$\Tilde{K}^h = S^{h^*}(K^h), \quad \Tilde{V}^h = S^{h^*}(V^h)$$

where $K^h, V^h$ are the original key and value matrices for head h. The sparsified caches $\Tilde{K}^h, \Tilde{V}^h$ are reused when computing attention for all subsequent timesteps.
\begin{algorithm}
\caption{KV-Malloc}
\label{alg:kvmalloc}
\begin{algorithmic}
\State {\bfseries Input:} $Q, K, V, t$ \Comment{Query, Key, Value, output position}

\State {\bfseries Output:} $\Tilde{K}, \Tilde{V}$ \Comment{Sparsified Key and Value}
\State {\bfseries Hyperparameters:} $S, \tau$ \Comment{Sparse schemes, similarity threshold}

\If{$t == 1$}
\For{$h=1$ {\bfseries to} $H$}
\State $A^h \gets$ Attention$(Q, K, V)$ \Comment{Compute attention}
\State $S^{h^*} \gets \argmax\limits_{k \in [1,m]} \text{sim}(A^h, S_k (A^h))$ \Comment{Select best scheme}
\EndFor
\EndIf

\For{$h=1$ {\bfseries to} $H$}
\State $\Tilde{K}^h \gets S^h(K^h)$
\State $\Tilde{V}^h \gets S^h(V^h)$ \Comment{Sparsify caches}
\EndFor

\State {\bfseries return} $\Tilde{K}, \Tilde{V}$
\end{algorithmic}
\end{algorithm}

\subsection{Eviction Policies}
In this section, we discuss the eviction policies used by KV-Malloc. The framework customize the eviction strategy for each head among the available ones. In our experiment, we implement 4 policies but the framework can be easily adapted to many more policies. More specifically, we include FOA, which is proposed by us, Locality, H20, and Average.

\textbf{Special Tokens}
FOA stands for First-of-All. This policy retains a mixture the KV values for the first token in the sequence, and the locality tokens at the current decoding position.

\textbf{Punctuation}
Locality refers to a strategy where only the KV pairs associated with the most recent tokens are retained.

\textbf{Frequency}
H2o keeps the values for a mixture of the estimated most important tokens and the most recent tokens.

\textbf{Locality}
Average keeps the average of values.



==> old_obs.tex <==
\label{sec:observation}
In this section, we present empirical observations that motivates our methods. We extract the attention scores of Llama 70B over random samples from GSM8k \cite{gsm8k} as an illustration.
% We first show the distinctive attention structures among attention heads in Section 3.1, which motivates our adaptive compression framework.
% In Section 3.2, we demonstrate that a single eviction policy cannot sufficiently capture the characteristics of all the head. 
% Then in Section 3.3, we show the profile of a head's attention structure tend to remain consistent over the whole decoding process, which inspires our one-sample profiling design.
\subsection{Head Distinctive Attention Structure}
\begin{figure}[h]
        \includegraphics[width=\textwidth]{figures/layers.pdf}
\caption{In this figure, we plot the dominant attention structure of each layer. For each layer, we calculate the number of heads having a significant portion of attention score contributed by the token type we classified in \ref{fig:obs}.  The Head Ratio, expressed as the fraction of heads predominantly attending to a specific token type relative to the overall number of heads.}
\label{fig:diverse}
\end{figure}
\textbf{Observation.} In \ref{fig:diverse}, we show the distinctive attention structures among neural modules.
We can see throughout the layers, the fraction of attention structures change dynamically.
For the initial and final layers, the attention is more evenly distributed to different token types. 
Conversely, in the middle layers, special tokens incrementally assert more dominance, while attention to other token types exhibits fluctuations.
At a closer look at each head in the same layer \ref{fig:obs}, we can see (1) the sparsity pattern is likely to differ among heads, (2) instead of single static token types, each head attends to a distinctive combination of token types.

\textbf{Insights.} The distinctive attention structure suggests that a single pattern \citep{h2o, scissorhands} may not have enough coverage. It could be beneficial to first diagnose the cache of each attention head before deciding how to construct the cache. We'll testify the benefit of this diagnose-to-compress strategy in the experiment section.
% We can see, for head 1 layer 3, a predominant mass of the attention, namely the darker blue cells in the figure, falls on the start token and the adjacent tokens while the other tokens are close to zero. 
% But for head 2 layer 3, we can observe the attention concentrates on special tokens like and ``$<s>$". 
% Overall, we can see the diversity nature of attention heads,despite being sparse.
% Inspired by \citeauthor{bert-look}, we hypothesize there are a limited set of frequent occurred attention patterns. We conclude 4 basic patterns based on manual inspections over the patterns on a wide range of tasks for both Llama and OPT.
% \begin{itemize}
%   \item FOA: FOA stands for First-of-All. This pattern mainly attends to the first token in the sequence, and the locality tokens adjacent the current decoding position.
%   \item H2O: a mix of heavy hitter tokens \citeauthor{h2o}, \citeauthor{scissorhands} and locality tokens.
%   \item Average.
% \end{itemize}
% We then show the percentage of the identified patterns in benchmarks.
% To approximate the fraction of each pattern, we hand-labeled approximately 400 instances into one of three distinct categories and a undecided category.
% This resulted in a somewhat skewed dataset, where the FOA category represented $40\%$ of the total heads. H2O take account for around $30\%$.
% Meanwhile, we would like to mention the summarized patterns are well generalized to fine-tune variations of foundation models. 
% We'll show the detailed coverage in Section 5.3.

% We can conclude (1) the sparsity pattern is likely to differ among heads, (2) the sparsity pattern types are consistently repeated among the 4 profiles. 
% The result motives us to design an adaptive KV cahce eviction strategy based on each specific head.
% The question remained is how to efficiently profile each attention head to decide its cache eviction policy. We show an interesting observation in the section below.

\subsection{Profile Tends to Be Consistent in One Sequence}
The previous section shows the potential benefit of a prior diagnosis for adaptive KV cache construction.
However, it's not clear how to design a diagnosis step , with sufficiently low overload, to guarantee the anticipated performance enhancement.

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/induction_1.pdf} % Replace with your image file
        \caption{Attention map at position 50}
        \label{fig:sub1}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/induction_2.pdf} % Replace with your image file
        \caption{Attention map at position 100}
        \label{fig:sub2}
    \end{subfigure}
    \\
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/induction_3.pdf} % Replace with your image file
        \caption{Attention map at position 150}
        \label{fig:sub3}
    \end{subfigure}
    \caption{Dominant attention distribution over the whole decoding sequence of Head 0 at Layer 16.}
    \label{fig:induction}
\end{figure}

\textbf{Observation} Fortunately, we find the profile of an attention head, tends to remain consistent through the decoding process.
We present an example in \ref{fig:induction}. We can see at when decoding the token at position 50 \ref{fig:sub1}, the head attends to mainly the special tokens, e.g., $<s>$ and $</s>$ at position 0 and 50 respectively, and tokens at 23, 28, etc.
This pattern is repeated at position 100 and 150.

\textbf{Insights.} The profile of each attention head can be consistent throughout the decoding process. To minimize the diagnosis overload, \ours only classifies the profiles once at the start of decoding. We'll testify how robust the design is in the experiment.

% \subsection{Profile a Head with One Step}
% \begin{figure}[h]
%         \includegraphics[scale=0.3]{figures/oneshot.png}
% \caption{The left figure shows attention distribution of 3 heads of the same layer at position 42. The right figure the perecentage of the identified five classes vs others.}
% \label{fig:oneshot}
% \end{figure}
% Our hypothesis is the head pattern tend to be persistent during the decoding.
% In our investigation, we posit that the behavior of attention heads exhibits temporal consistency throughout the decoding process. Specifically, if an attention head is classified as focusing on a particular aspect, such as First Order Attention (FOA), during the initial step of decoding, it is highly probable that it will maintain this FOA classification throughout subsequent decoding steps. 
% To articulate this formally, it is a reasonable approximation to consider that the attention profile of a head across all decoding steps can be reliably predicted by its profile established at the inaugural decoding step.
% To empirically verify this, we sample 400 instance of attention heads of Llama when doing inference on Bigbench.
% We show in \ref{fig:oneshot} that most of the heads remain a persistent profile throughout the generation process.


==> old_related.tex <==
\textbf{Attention Pattern Analysis} 
Several studies have sought to understand the roles individual attention heads play in the Transformer. 
\cite{lift-prune} analyzed the self-attention heads in BERT \cite{bert} using LRF \cite{lrf} and characterize them into interepretable roles, one of which is to attend to adjacent tokens all the time.
\citeauthor{sixteen} found even heads in the same layer could have different impact on the performance while the importance of individual head change across tasks.
\citeauthor{bert-look},\citeauthor{dark} found a significant portion of heads attends separator tokens, next or previous tokens and a hybrid of them. 
We observe consistent patterns in decoder-only models, despite previous studies are mainly done on encoder models. 
Our work shares similar spirits of these studies, 
% in terms of capturing the diversity and coherence among attention heads, 
but we focus on characterizing the KV cache of individual head. 
% Several studies have sought to understand the roles individual attention heads play in the Transformer. 
% \cite{lift-prune} analyzed the self-attention heads in BERT \cite{bert}, finding that different heads could attend to various, highly specialized semantic and linguistic concepts. 
% \citeauthor{sixteen} found that some heads focus on semantic meaning while others could track positional information. 
% \citeauthor{bert-look} has developed methods to quantify the extent to which attention heads exhibit syntactic, semantic, or positional biases. 
% \citeauthor{dark}, \citeauthor{head-ling} visualized attention to study the emergence of linguistics structures.

\textbf{Efficient Transformer}
This line of work can be roughly categorized into computation-efficient attention approximation, network compression techniques, KV cache optimization.


Computation-efficient attention approximation mainly leverages sparse and low-rank approximation to reduce the computational complexity of self-attention \citeauthor{sparsetransformer}, \citeauthor{lineartrans}, \citeauthor{reformer}.

Network compression techniques such as pruning, quantization, and knowledge distillation have been widely studied to reduce the size of neural networks. Quantization and distillation are orthogonal to our method but can be compatible to integrate in the future.
% Quantization uses lower precision weights to compress models without significantly impacting accuracy \citeauthor{deepcomp}, \citeauthor{intquant}, \citeauthor{dfquant}. 
% Distillation transfers knowledge from a large teacher model to a smaller student model \citeauthor{hintdistill}, \citeauthor{distbert}. 
% These two directions are orthogonal to our method but can be compatible to integrate in the future.

Pruning removes redundant weights and connections in the model, which can be roughly categorized into unstructured and structured. Unstructured pruning removes individual weight based on certain numerical like magnitude \citeauthor{magaprune}, gradient movement \citeauthor{moveprune}, \citeauthor{secondprune}, lottery hypothesis\citeauthor{lottery}. 
These methods are rarely used in practice due to their poor compatibility with modern accelerators.
Structured pruning\citeauthor{structureprune} works on a relative coarse granularity, eliminating the whole set of parameters from the model. \cite{sixteen}, \citeauthor{lift-prune} proposes methods to remove unimportant heads determined by weights and loss perturbations.
\citeauthor{deebert} proposes to discard following attention layers following predictions of an extra classification module. 
\citeauthor{tileprune}, \citeauthor{blockprune}, \citeauthor{blockprune} investigate sparse factorization method to decide structures to be pruned.
Overall, these methods works on the model weight side. We study a different bottleneck, the KV cache, which is larger and more dynamic compared to the weights itself.
% these methods require heavy additional training during or after pruning, without which will cause significant performance regression \citeauthor{danqiprune}.
 
In the KV cache literature, there are a few concurrent work exploring similar topics. \citeauthor{h2o} proposes an eviction policy to retain a combination of recent tokens and important tokens decided by frequency statistics. However, their methods requires expensive sorting at each step to prevent significant performance degradation otherwise. \citeauthor{scissorhands} similarly proposes a frequency-based criteria to decide pivot tokens to be retained in cache. The focus of our work is to capture the intrinsic mechanics of each attention head, and adaptively decide the eviction policy.

